Approximation Algorithms for Multi-Robot Patrol-Scheduling with Min-Max Latency

We consider the problem of finding patrol schedules for $k$ robots to visit a given set of $n$ sites in a metric space. Each robot has the same maximum speed and the goal is to minimize the weighted maximum latency of any site, where the latency of a site is defined as the maximum time duration between consecutive visits of that site. The problem is NP-hard, as it has the traveling salesman problem as a special case (when $k=1$ and all sites have the same weight). We present a polynomial-time algorithm with an approximation factor of $O(k^2 \log \frac{w_{\max}}{w_{\min}})$ to the optimal solution, where $w_{\max}$ and $w_{\min}$ are the maximum and minimum weight of the sites respectively. Further, we consider the special case where the sites are in 1D. When all sites have the same weight, we present a polynomial-time algorithm to solve the problem exactly. If the sites may have different weights, we present a $12$-approximate solution, which runs in polynomial time when the number of robots, $k$, is a constant.

==> buggy-weighted.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%====================== %%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Min-Max weighted latency in metric space}
\rey{This subsection need to rewrite. Right now it only fits when k=1, which is not interesting.}

There is a connection between the $k$-robot patrol scheduling problem and the time window travelling salesman problem with $k$ robots ($k$-TWTSP).

\begin{definition}[$k$-TWTSP~\cite{gaoapproximation}]
The $k$-robot time-window TSP problem ($k$-TWTSP) asks for a
path $\sigma_i$ for each robot $r_i$ such that all the sites are visited within their respective time windows ($[a_j, b_j]$ for site $j$). Given the speed bound of $v \geq v_{min}$, where $v_{min}$ is the smallest speed such that there exists a feasible solution, the objective is to minimize the sum of the lengths of all paths.
\end{definition}

\begin{definition}[Dual approximation algorithm for $k$-TWTSP~\cite{gaoapproximation}]
Given an instance of $k$-TWTSP problem in a metric space with metric
$d(\cdot , \cdot)$, let $D$ be the total travel distance of all robots in the optimal solution travelling with a feasible speed $v$. An algorithm is an $(\alpha, \beta)$ dual approximation if every robot moves with speed at most $\alpha v$; and the robots travel a total distance at most $\beta D$. 
\end{definition}

In~\cite{gaoapproximation} there is an $(\alpha, \beta)$-dual approximation algorithm to the $k$-TWTSP when the time windows are dyadic intervals (a dyadic interval is of length as a power of two and the left endpoint is a nonnegative integer multiple of its length, e.g., $[m2^j, (m+1)2^j]$, for some $m\geq 0$, $j\geq 0$), with $\alpha=O(\log \ell_{max})$, $\beta=O(\log \ell_{max})$, where $\ell_{max}$ is the maximum time window length (the minimum window length is assumed to be $1$). We will use this algorithm to solve our $k$-robot patrol scheduling problem.

Given an instance of $n$ sites with weight $w_i$ for site $s_i$ in a metric space, we assume all distances are integer values\footnote{In general, we can approximate the distances using  a $1+\eps$ approximation by rational numbers, with $\eps>0$ arbitrarily close to $0$.}. Suppose $L$ being the optimal latency of the $k$-robot patrolling problem, we formulate a $k$-TWTSP problem. First, we set the time windows for the sites. For the site $s_i$ with weight $w_i$, the length of its time window is defined as $\ell_i = L/w_i$. We now fix the unit of time to be the smallest time window size, i.e., $L/w_{max}$, where $w_{max}$ is the largest weight of all sites. The largest time window becomes $\ell_{max}=w_{max}/w_{min}$.
Then we relax each time window length to the least upper bound of ``dyadic'' values. That is, $\ell'_i=\sup \{2^x | x \in \mathbb{N} \text{ and } 2^x \geq \ell_i \}$. 
Clearly $\ell'_i\leq 2\ell_i$.
Define $\ell'_{max}=\max_i {\ell'_i}$. 
Each site $s_i$ is mapped to a set $A_i$ of $\tau_i = N \cdot \ell'_{max} / \ell'_i$ new sites, i.e. 
    $A_i=\{ a_{i1},a_{i2},\dots a_{i{\tau_i}} \}$, where $N$ is a big integer to be determined later. 
In addition, each site $a_{iy}\in A_i$ is located at site $s_i$ and has a time-window constraint $[y \ell'_i,  (y+1)\ell'_i]$. These time windows are dyadic intervals. 
In fact, for each site $s_i$ the time windows for the new sites in its corresponding set $A_i$ together cover the entire time interval of $[0, T]$, with $T=N \cdot \ell'_{max}$.

Since $L$ was assumed to be the optimal latency of the $k$-robot patrol scheduling problem, the $k$-TWTSP above has a feasible solution when the robots travel with maximum speed of $1$, i.e., all time windows are hit.  

Now, assume we magically know the value of $L$ and formulate the $k$-TWTSP problem as above, the algorithm in~\cite{gaoapproximation} finds a $k$-TWTSP solution consisting of $k$ paths $\{C_1, C_2, \cdots, C_k\}$ in which robots moving with speed $\alpha=O(\log \ell'_{max})$ (with $r_i$ along $C_i$) meet the specified time windows. We now turn the paths $\{C_1, C_2, \cdots, C_k\}$ into a patrol schedule for the $k$-robot patrol problem. 

First, we turn the paths into a periodic schedule. Our robots move either with full speed of $1$ or stop for an integer amount of time at a site. For each site pair $s_i, s_j$, the time taken for a robot to travel from $s_i$ to $s_j$ is precisely $d(s_i, s_j)$. We can imagine adding $d(s_i, s_j)-1$ dummy sites, uniformly placed between $s_i, s_j$. The distances between these dummy sites and $s_i, s_j$ are integers. Therefore, for any integer time $t$ in $[0, T]$, let $C_i(t)$ refer to the location of robot $r_i$ at time $t$. $C_i(t)$ is either at a site or a dummy site. The total number of sites and dummy sites is $M=\sum_{ij} d(s_i, s_j)$.
We define a status vector of the $k$ robots at integer time $t$, $t=0, 1, 2, \cdots, T$, as a $k$-dimensional vector
$$V(t)=\{C_1(t), C_2(t), \cdots, C_k(t)\}.$$
Notice that the vector $V(t)$ is a discrete vector of a total $M^k$ possible values. Therefore, if we take $T$ larger than $M^k$, the status vector will necessarily repeat itself. Assume that the status vectors at integer time $j_1$ and $j_2$ are the same. We let robot $r_i$ follow path $C_i(j_1)$ till $C_i(j_2)$ and repeat infinitely. In this schedule, each site is visited with maximum latency at most $2\alpha\ell'_i \leq 4 \alpha\ell_i$, since the robots move at unit speed (instead of the accelerated speed of $\alpha$). This solution gives a maximum weighted latency at most $4\alpha \ell_i w_i =4\alpha L$, thus being an $O(\log(w_{max}/w_{min}))$-approximation.

Since we do not know the optimal value $L$, we just use a value $L_0 \geq L$, for example, take $L_0$ to be the maximum weighted latency of $k$ robot following a TSP tour. Suppose $L_0=\gamma L$ for a value $\gamma>1$. The formulated $k$-TWTSP problem using $L_0$ is simply a scaled version of the problem using $L$ with the combinatorial structure unchanged. Thus the minimum speed $v_{min}$ needed for the $k$-TWTSP problem using $L_0$ admitting a feasible solution is basically $1/\gamma$. Since we ask the robots to travel in unit speed, the formulated problem using $L_0$ must be feasible. Thus the approximation factor of  
$O(\log(w_{max}/w_{min}))$ holds in the same manner. The running time is polynomial in $M^k$, $n$, and $w_{max}/w_{min}$.

\begin{theorem}
Given $n$ sites with weight $w_i$ for site $s_i$ in a metric space, one can compute a patrol schedule of $k$ robots with approximation factor of $O(\log(w_{max}/w_{min}))$ for minimizing the maximum weighted latency of the sites. The running time of the algorithm is polynomial in $M^k$, $n$, and $w_{max}/w_{min}$, where $M$ is the sum of all pairs distances.  
\end{theorem}

==> periodicity.tex <==
\subsection{Basic Properties}


Since the problem asks for an infinite sequence, we need to first show that the problem is well defined. First, we can take any traveling salesman tour of length $L_0$ and place $k$ robots uniformly on the tour to generate finite latency of $L_0/k$ for all sites. So the minimum latency is at most $L_0/k$ and cannot be infinite. 

\begin{lemma}
If the distances between all sites are rational, there is an optimal solution that is periodic, i.e., for a schedule $\Sigma=\{\sigma_1, \sigma_2, \cdots, \sigma_k\}$, there is a finite sequence $\Delta(\Sigma)$ such that $\Sigma$ is constructed by repeating $\Delta(\Sigma)$ infinitely many times. 
\end{lemma}
\begin{proof}
Without loss of generality we can assume that all distances are integer values, since multiplying all distances by a large constant does not change the combinatorial nature of the solution. Now we take one optimal solution $\Sigma=\{\sigma_i\}$ with latency $L$. 


Since all distances are integer values, we can consider time as slotted at integer values. \jie{what if a robot waits for an irrational amount of time?} 



Take a time slot $j> L_0/k$, the current status of the $k$ robots can be represented by a $k$-tuple $\{(v_{i,j}, t_{i,j})\}$: the robot $r_i$ will arrive at $s_{i,j}$ after $t_{i,j}$ slots. Notice that $s_{i, j}$ is one of the $n$ sites and $t_{i, j}$ is an integer at most $L'$, thus being finite. The total number of possible $k$-tuples for the status of the $k$ robots is finite. 

Now we consider the family $U$ of sub-schedules of length within $L'$, represented by the sequence of robot status tuples. Each of them covers all sites in $P$.
Again there are only a finite number of different sub-schedules.
Since the schedule $\Sigma$ is infinitely long, there must be a sub-schedule $\Sigma_1$ from time $t_1$ to $t_2$ that repeats itself later in the schedule, say, from time $t_3$ to $t_4$, $t_1< t_2 < t_3 < t_4$. Define $W_2$ as $\Sigma(t_2+1, t_3-1)$. Concatenate $W_1$ and $W_2$ and then wrap it around to form a periodic schedule $\Sigma'={W_1, W_2, W_1, W_2, \cdots}$. We can now argue that $\Sigma'$ is also optimal.

Consider two consecutive visits to the same site $s$ in $\Sigma'$. One of the following two cases must be true: They appear in either consecutive appearances of $W_1$ followed by $W_2$, or consecutive appearances of $W_2$ followed by $W_1$. In either case this instance appears in $\Sigma$ and thus the latency is no greater than the optimal latency $L$. Thus the claim is true.
\end{proof}

%Assume otherwise, there does not exist a solution of minimum latency. There can only be two possibilities for this to happen. Either all possible solutions by the $k$ robots have maximum latency to be infinite, or there is an infinite sequence of solutions $S_1, S_2, \cdots$ with latency $F_1, F_2, \cdots$ such that $\lim_i F_i=F$ but no solution reaches $F$. The former is clearly not true -- since we can take any traveling salesman tour and place $k$ robots on the tour to generate a finite latency for all sites. Let's suppose the maximum latency of this solution to be $F_0$. For the latter case, we show that there are only a finite number of different values smaller than $F_0$ that can be the latency of the $k$-robot solutions. First, for any site $p$, there is a finite number of sequences beginning in $p$ with total length less than $F_0$, since all distances are positive. Hence, there is a finite number of possible latency values for site $p$ that are less than $F_0$.  Since there is a finite number of $n$ sites, there cannot be an infinite sequence of values which approaches $F$ but never reaches $F$. Therefore, the claim is true.

If the distances are not rational, we can approximate the distances by rational values with approximation up to $1+\eps$, for any $\eps>0$. 

When $k=1$, even if the sites carry different weights for respective latency, it is known that there must be an optimal periodic solution for any metric space~\cite{alamdari2014persistent} -- since the issue of synchronization among the robots no longer matters. 
\jie{Can we find an example for $k\geq 2$ when there is no periodic optimal solution?}

==> weighted-metric.tex <==

%=================== General case ===================

%subsection{Min-Max Weighted Latency in General Metric Setting}
%Compared with Section~\ref{sec:weighted in 1D}, there are two key differences that makes the general metric much harder. First, the path of a robot cannot record as a leftmost and rightmost positions (or at least, constant positions) such that every site between this interval is free to visit. Secondly, robots may move under many different paths rather than along a line. Thus, we cannot use the exchange argument for robots and have to take the synchronization of robots into consideration.
%\subsection{$O(k\log n)$-Approximation in General Metric Setting}

\subsection{$O(k\frac{w_{\max}}{w_{\min}})$-Approximation in General Metric Setting}

For sites with weights in a general metric $d$, we design an algorithm with approximation factor $O(km)$ for minimizing the max weighted latency of all sites by using $k$ robots of maximum speed of $1$, where $m$ is the ratio of the maximum weight to the minimum weight. The intuition of our algorithm is the following. We first guess an upper bound $L$ on the optimal maximum weighted latency and see if we can construct a schedule such that the maximum weighted latency is no greater than $O(km)L$. If not, we double the value of $L$ and run again. We prove that if we cannot construct a schedule that has latency $O(km)L$ with this algorithm then the optimal latency must be greater than $L$. Thus, when we successfully find a schedule, it will be one with maximum weighted latency as an $O(km)$ approximation to the optimal. Additionally, if the maximum distance between sites is bounded, we can slightly modify the algorithm to have a $O(k\log n)$ approximation.

Without loss of generality, we assume that the maximum weight among sites is 1. Similar to the previous section, we first round the weight of each site to the least dyadic value and solve them problem with dyadic weights. This will only introduce another factor of $2$ in the approximation factor on the maximum weighted latency. 

Denote by $\{W_1,W_2, \cdots W_m \}$ the collections of sites where $W_j=\{s_i |\ w_i = 1/2^{j-1} \}$ and $W_j$ could be empty.
%, if there are no sites with weights within $[1/2^{j}, 1/2^{j-1})$. 
Also $\beta$ is the approximation factor of a min-max tree cover algorithm $\mathcal{A}$, the best known of which is $8/3$~\cite{xu2013approximation}.
$L$ is a parameter. 
%We define the distance between two trees as the shortest distance between nodes that belong to different trees. 
Now, we introduce two algorithms:
\begin{itemize}
    \item Algorithm \textsc{$k$-robot assignment}($\{ W_j \},L$), returns \textsc{False} when there does not exist a schedule with max weighted latency $\leq L$, or, returns a group of trees $\mathcal{T}_i$ for each robot $r_i$ such that no site belongs to two trees. Among the trees assigned to robot $r_i$, one of the tree is called  a depot tree and one vertex on the depot tree is a \emph{depot} for $r_i$. With these trees $\mathcal{T}$ assigned to one robot, the procedure
    \item Algorithm \textsc{Single Robot Schedule}($\mathcal{T}$) returns a single-robot schedule such that every site covered by $\mathcal{T}$ has maximum weighted latency $O(km \cdot L)$.
\end{itemize}
Clearly, the two procedures together provide what is needed. 

Denote $V(T)$ the set of vertices of a tree $T$ and $d(s_1, s_2)$ the distance between two sites $s_1$ and $s_2$. 

\smallskip
\noindent\fbox{\scalebox{0.97}{\begin{minipage}{\textwidth}
\begin{algorithmic}[1]
  \Procedure{$k$-robot assignment}{$\{ W_j \},L$}   %\Comment{Find a schedule for $k$ robots such that the max weighted latency is at most $O(k\log n)L$, or return \textsc{False} when no schedule can have max weighted latency $\leq L$.}
  \For{every set $W_j$}
    \For{$t=1$ to $k$} 
        \State Run algorithm $\mathcal{A}$ to obtain the $t$-min-max tree cover $\mathcal{C}^j_t$ on $W_j$.
    \EndFor
    \State $q_j \leftarrow$ smallest integer $t$ s.t. the max weight of trees in $\mathcal{C}^j_t$
    is $< \beta \cdot 2^{j-1} L$. 
    \State Only keep the trees in the $q_j$-min-max tree cove: $T^j_1, T^j_2, \cdots T^j_{q_j}$.
    \State If there is no such $q_j$, Return \textsc{False} \label{algo:k-robot-schedule_first return false}
    \EndFor
  \State Set all robots as ``free'' robots, i.e., not assigned a depot tree.
  \For{$j$ from 1 to $m$} \Comment{Assign trees to robots}
    \For{$i$ from 1 to $q_j$}
        \State $Q\leftarrow V(T^j_i)$.
        \For{every non-free robot $r$} 
            \State $T^{j'}\leftarrow$ the depot tree of $r$
            \State $x\leftarrow$ the depot vertex $x$ of $T^{j'}$
            \State $Q' \leftarrow \{v| v\in Q, d(v,x) \leq 2^{j'-1}L \}$
            %and $dist$ is the distance function.
            \State Compute $\MST(Q')$ and assign it to robot $r$.
            \State $Q \leftarrow Q \setminus Q'$. 
        \EndFor
        \If $Q\neq \emptyset$ 
             \If{no free robot} 
        %(being too far from depot trees and there is no free robot), 
         \State Return \textsc{False}.
        \Else 
        \State Assign $\MST(Q)$ as the depot tree of a free robot and take an arbitrary vertex in $Q$ as the depot.
        \EndIf
        \EndIf
    \EndFor
  \EndFor
  \State Return the group of trees, $\mathcal{T}_i$, assigned to robot $r_i$, $\forall i$
\EndProcedure
\end{algorithmic}
\end{minipage}}}
\smallskip
%\ben{The above algorithm block is very long and the tabbing is hard to read, also it is causing issues with the previous page.}

A few quick observations are obvious about the distances of two sites on different depot trees, or on trees assigned to the same robot.

%\jie{There is still a bug. For a site $s$ in the second depot tree $T_2$, it cannot be assigned to a previous depot tree $T_1$ -- meaning that there is a site $s'$ in $T_1$ such that $s, s'$ are far away. But this does not mean that $s$ is far away from every site on $T_1$. So the following lemma is still problematic.}

\begin{lemma}\label{lem:far-away-different-depot-trees}
In \textsc{$k$-robot assignment}($\{ W_j \},L$), the depot $s_i$ and $s_j$, with $w_i\geq w_j$, for different robots have distance more than $L/w_i=2^{j-1} L$.
\end{lemma}
\begin{proof}
Since $s_i$ and $s_j$ are depot vertices belong to different robots, the nodes in the second depot tree (the one what is created later in order) must be ``far away'' from the first depot, i.e., of distance more than $L/w_i$ away. Thus any two sites of the two trees are of distance  more than $L/w_i$ away. 
\end{proof}

%\begin{lemma}
%In \textsc{$k$-robot assignment}($\{ W_j \},L$), two sites $s_i$ and $s_j$, with $w_i\geq w_j$, from different trees assigned to the same robot $r$, have distance at most $L/w_i$.
%\end{lemma}

\begin{lemma}
\label{lem: L leq L_star}
Given $L$, if \textsc{$k$-robot schedule}($\{ W_j \},L$) returns \textsc{False} then $L<L^*$, where $L^*$ is the optimal maximum weighted latency.
\end{lemma}
\begin{proof}
There are two cases of the algorithm returning \textsc{False}. We discuss them separately.

In the first case, there is a value $j$ such that the maximum tree weight of a $\beta$-approximation of the $t$-min-max tree cover is larger than $\beta 2^{j-1} L$ for all $1\leq t\leq k$.
It implies that the optimal value $\lambda$ of $k$-min-max tree cover is larger than $2^{j-1} L$ for sites in $W_j$. Since the $k$-robot solution also cover all the sites in $W_j$, $\lambda/2^{j-1}$ is also a lower bound of the optimal latency (see Section~\ref{subsec: appetizer approximation algorithms}). Thus, we have, $L^* \geq \frac{1}{2^{j-1}}\lambda > \frac{1}{2^{j-1}} 2^{j-1} L =L$.

In the second case, there is a tree with vertices that are far away from existing depots and there is no free robot anymore. Notice that there are precisely $k$ depots at this moment. Suppose the depots are $s_1,s_2, \cdots s_k$ and there is another depot vertex $s_{k+1}$ that is far away from the $k$ depots. 
In fact, we claim the following. For any $p$ sites $\subseteq \{s_1,s_2, \cdots s_k \}$, there must be $p$ robots to serve these sites; otherwise one of the sites has weighted latency more than $L$. This will be sufficient for our claim as we have $k+1$ depots and only $k$ robots.

Suppose we have $p$ depot sites $s_1,s_2, \cdots s_p$ from $p$ depot trees respectively. We first prove the claim when these sites are in $W_j$ for some $j$.  In this case, any two of the $p$ sites are of distance more than $2^{j-1} L$ away.
Take the optimal schedule of $p-1$ robots that minimize the maximum latency in sites $\{s_1,s_2, \cdots s_p\}$. Given a time $t, t>0$, each robot must be either on one of the sites or moving towards a site. We say a robot is ``claimed'' by site $s$ at time $t$ if the robot is either at $s$ or moving towards $s$. One robot can only be claimed by one site. Since there are $p$ sites but only $p-1$ robots, there must be a site $s$ that has not been assigned any robot. Thus, the latency of $s$ is larger than $L$ since the distance from any other sites to $s$ is larger than $2^{j-1} L$.

\begin{figure}[h]
      \centering
      \includegraphics[scale=0.9]{figs/balls-robots.pdf}
      \caption{An example of $s_1,s_2,s_3$ with weights $w_1>w_2>w_3$ and two robots $r,r'$. Balls with center $s_1,s_2,s_3$ have radii $L/w_1,L/w_2,L/w_3$ respectively. Since $r,r'$ are claimed by $s_1,s_2$ respectively; there is no robot for $s_3$ to claim. Thus the weighted latency must be more than $L$.}
      \label{fig:balls-robots}
\end{figure}

Now we prove the claim when the sites may have different weights. Suppose the sites $s_1,s_2, \cdots s_p$ have decreasing weights $w_1 > w_2> w_3> \cdots, > w_p$ and there are only $p-1$ robots to serve these sites. By Lemma~\ref{lem:far-away-different-depot-trees}, two sites $s_i$ and $s_j$, with $i<j$, are from different depot trees and thus their distance is more than $L/w_i$. We draw a ball $B(s_1,L/w_1)$ with the center at $s_1$ and radius $L/w_1$. No other sites are within this ball. Similarly, no other sites, except $s_1$ are in the ball $B(s_2,L/w_2)$. An example of three sites is shown in Figure~\ref{fig:balls-robots}.

Now, assume the optimal schedule gives a minimum weighted latency less than $L$. At any time $t$ in the schedule, there must be a robot $r$ that is claimed by $s_1$ and this robot must stay within the ball $B(s_1,L/w_1)$; otherwise, no robot can visiting $s_1$ during the time interval $[t,L/w_1]$, i.e., the weighted latency of $s_1$ would be more than $L$. With the same argument, there must exist a robot $r'$ that stays within $B(s_2,L/w_2)$ and $r'$ is claimed by $s_2$. Notice that $r'$ cannot be the same robot as $r$ since $r$ always stays within $B(s_1,L/w_1)$ and cannot visit $s_2$ which is outside of $B(s_1,L/w_1)$.
Apply the same argument, 
the first $p-1$ sites $s_1, s_2, \cdots, s_{p-1}$ each claim a different robot and there is no robot left to serve $s_p$. Thus, the optimal weighted latency is more than $L$. 
\end{proof}

\begin{lemma}\label{lem:short-distance} 
If \textsc{$k$-robot schedule}($\{ W_j \},L$) does not return \texts{False}, each robot is assigned a set of at most $km$ trees and a depot site such that 
\begin{itemize}
    \item one of the trees is a depot tree $T^j$, say, with vertices from $W_j$;
    \item all other vertices are within distance $\beta 2^{j-1}L=\beta L/w_i$ from the depot site.
\end{itemize}
\end{lemma}
\begin{proof}
Most of the claim is straight-forward from the algorithm \textsc{$k$-robot schedule}($\{ W_j \},L$). The only thing to prove is the number of trees assigned to a robot. 
There are at most $km$ trees obtained from the min-max tree cover on all sites $W_1, W_2, \cdots, W_m$. The vertices of a single tree might be allocated to some non-free robots and each robot is assigned by at most one subset of the vertices. Thus for a single robot $r$, there is a depot tree $T^j$ and at most $km$ additional trees.
\end{proof}

Now we are ready to present the algorithm \textsc{Single Robot schedule}($\mathcal{T}$) for finding the schedule for robot $r_i$ to cover all vertices in the family of trees $\mathcal{T}_i$, as the output of \textsc{$k$-robot schedule}($\{ W_j \},L$). Below we present the details. Suppose there is a family of $h$ trees $\mathcal{T}$ among which $T_1$ is the depot tree. 

\smallskip

\noindent\fbox{\scalebox{0.97}{\begin{minipage}{\textwidth}
\begin{algorithmic}[1]
  \Procedure{Single Robot Schedule}{$\mathcal{T}=\{T_1, T_2, \cdots, T_h\}$}   
    %\State According to the order of tree assignments for $r_i$, denote by $D_1,D_2, \cdots D_\eta$ the tours that traverse each tree with shortcuts ($D_1$ is the tour for the depot tree of $r_i$). 
    \For{$i=1$ to $h$} 
    \State Compute tour $D_i$ by traversing $T_i$ with possible shortcuts. 
    \EndFor
    \State $\delta\leftarrow |D_1|/2$.
    \State $i\leftarrow 1$.
    \For{$i=1$ to $h$}
        \State $p_i\leftarrow$ an arbitrary site on $D_i$.
    \EndFor
    $i\leftarrow 1$
    \While{Not all sites are covered}
        \State Walk on $D_i$ for distance $\delta$ and arrive at $p'_i$
        \State $p_i\leftarrow p'_i$.
        \State $i\leftarrow i+1$.
        \State If $i>h$, $i\leftarrow 1$.
        \State Robot moves to $p_{i}$. 
    \EndWhile
\EndProcedure
\end{algorithmic}
\end{minipage}}}

\begin{lemma}
The \textsc{Single Robot schedule}($\mathcal{T}=\{T_1, T_2, \cdots, T_h\}$) returns a schedule for one robot that covers all sites included in $\mathcal{T}$ such that the maximum weighted latency of the schedule is at most $O(km)\cdot L)$.
\end{lemma}

\begin{proof}
By Lemma~\ref{lem:short-distance} the distance between the depot and any vertex on tree $T_i$ is at most $\beta L/w_i$. By triangle inequality, the distance of any two sites on tree $T_i$ and $T_j$ respectively is at most $2\beta L/w_i$. 
%\jie{Here is the bug. Although the smallest distance between the two tours is at most $O(D_1)$ away but the tours $D_x$, $D_y$ can be much longer. So when the robot jumps from one tour to another, the distance is not necessarily in the order of $D_1$} 
Consider a site $s$ on $D_i$. There are two cases; if $|D_i| > \delta$, the time of any consecutive visits to $s$ is 
$$
O( \ceil[\bigg]{ \frac{|D_i|}{\delta} } \cdot (|D_1|+\delta) \cdot h )=O(2^{j-1}L \cdoth ).
$$
Since there are at most $km$ trees the weighted latency of $s$ is $O(kmL).$ On the other hand, if $|D_i| \leq \delta,$  the time of any consecutive visits to $s$ is 
$
O(|D_1| \cdot km)=O(2^{j'-1}L \cdot km),
$ where $j'\leq j$. Thus, the weighted latency is also $O(kmL)$.
\end{proof}

If the maximum distance between sites is bounded, we can modify the algorithms to have a $O(k\log n)$ approximation. The process is similar with the proof in Bamboo Garden Trimming Problem (BGT)~\cite{lingasbamboo}. We slightly modify the definition of $W_m= \{ s_i|\ w_i \leq 1/n^2 \}$. The algorithms are also slightly modified for sites in $W_m$. In \textsc{$k$-robot assignment}, we do not build min-max tree cover for set $W_m$ but only one minimum spanning tree for $W_m$. The algorithm does not return False if this tree has weight larger than $L$. In \textsc{Single Robot schedule}, for a single robot, if the vertices of the last tour $D_h$ are from the collection of sites $W_m$, instead of walking on $D_h$ for distance $\delta$, the robot walks only a site in $D_h$.

With the modification of the algorithms, Lemma~\ref{lem: L leq L_star} and Lemma~\ref{lem:short-distance} still hold. There are at most $\log n $ groups of sites (i.e., $m=O(\log n)$). For sites in set $W_j\ j \neq m$, the weighted latency is the same as the above analysis, which is $O(kmL)=O(k\log n L)$. For site $s$ in set $W_m$, the time of any consecutive visits is 
$$
O(|W_m|\cdot  |D_1| \cdot h)=O(n|D_1| \cdot k\log n ),
$$
where $|W_m|$ is the number of sites in $W_m$. Since $s$ has weight at most $1/n^2$ and $|D_1|= O(n)$ , the weighted latency of $s$ is $O(k\log n)$. Thus, the weighted latency for all sites is $O(k\log n L)$.

\begin{corollary}
If the distance between sites are bounded, by slightly modifying \textsc{$k$-robot assignment} and \textsc{Single Robot schedule}, we can have an algorithm with $O(k\log n)$ approximation.
\end{corollary}

